An Order Theory Framework of Recurrence Equations for Static Cost Analysis $-$ Dynamic Inference of Non-Linear Inequality Invariants

Recurrence equations have played a central role in static cost analysis, where they can be viewed as abstractions of programs and used to infer resource usage information without actually running the programs with concrete data. Such information is typically represented as functions of input data sizes. More generally, recurrence equations have been increasingly used to automatically obtain non-linear numerical invariants. However, state-of-the-art recurrence solvers and cost analysers suffer from serious limitations when dealing with the (complex) features of recurrences arising from cost analyses. We address this challenge by developing a novel order-theoretical framework where recurrences are viewed as operators and their solutions as fixpoints, which allows leveraging powerful pre/postfixpoint search techniques. We prove useful properties and provide principles and insights that enable us to develop techniques and combine them to design new solvers. We have also implemented and experimentally evaluated an optimisation-based instantiation of the proposed approach. The results are quite promising: our prototype outperforms state-of-the-art cost analysers and recurrence solvers, and can infer tight non-linear lower/upper bounds, in a reasonable time, for complex recurrences representing diverse program behaviours.

==> table_of_benchmarks.tex <==
{\footnotesize
 \renewcommand{\arraystretch}{2}%
\begin{longtable}[c]{| c | c | c | p{5.5cm} | p{4.8cm} |}
\caption{Benchmarks\label{table:benchmarks}}\\
\hline
\multicolumn{3}{|c|}{\textbf{Bench}} %
& \makecell[c]{\textbf{Equation}} & \makecell[c]{\textbf{Solution}} \\ \cline{1-5} \cline{1-5}
\endfirsthead
\caption[]{Benchmarks (continued)}\\
\cline{1-5}
\multicolumn{3}{|c|}{\textbf{Bench}} %
& \makecell[c]{\textbf{Equation}} & \makecell[c]{\textbf{Solution}} \\ \cline{1-5} \cline{1-5}
\endhead
\multirow{7}{*}{\rotatebox[origin=c]{90}{\texttt{\catwithnoise}}}
 & \texttt{\runningexname}
 & \texttt{\runningexkey}
 & \gape{\scalebox{0.7}{$f(n,c)=\begin{cases*}
      f(n-1, 0)   + n + 300 & if $n>0 \wedge c\geq 100$\\[-2pt]
      f(n-1, c+1) + n       & if $n>0 \wedge c <   100$\\[-2pt]
      c                     & if $n=0$\\
    \end{cases*}$}}
 & \gape{\scalebox{0.7}{$\begin{cases*}
      \frac{n(n+1)}{2} + n + 299 + 199\lfloor\frac{n-1}{101}\rfloor\\
           \qquad \text{ if } n>0 \wedge c\geq 100\\[-2pt]
      \frac{n(n+1)}{2} + n + c + 199\lfloor\frac{n+c}{101}\rfloor\\
           \qquad \text{ if } n>0 \wedge c <   100\\[-2pt]
      c    \qquad\!\!\! \text{ if } n=0
    \end{cases*}$}}
 \\ \cline{2-5}
 & \texttt{\noiseddtwotwoname}
 & \texttt{\noiseddtwotwokey}
 & \gape{\scalebox{0.7}{$f(n,c)=\begin{cases*}
      f(n-1, 0)   + n + 300n & if $n>0 \wedge c\geq 100$\\[-2pt]
      f(n-1, c+1) + n        & if $n>0 \wedge c <   100$\\[-2pt]
      c                      & if $n=0$\\
    \end{cases*}$}}
 & \gape{\makecell[l]{
     \scalebox{0.7}{Hard to express exactly, but}\\
     \scalebox{0.7}{for $c\geq 100$, and $n\to\infty$,}\\
     \scalebox{0.7}{$=\frac{n(n+1)}{2}+\frac{300}{101}\frac{n(n+101)}{2} + \rO(1)$}
     }}
 \\ \cline{2-5}
 & \texttt{\fillandfreename} 
 & \texttt{\fillandfreekey} 
 & \gape{\scalebox{0.7}{$f(n,c)=\begin{cases*}
      f(n-1, 0)   - c & if $n>0 \wedge c\geq 99$\\[-2pt]
      f(n-1, c+1) + 1 & if $n>0 \wedge c <   99$\\[-2pt]
      0               & if $n=0$\\
    \end{cases*}$}}
 & \gape{\scalebox{0.7}{$\begin{cases*}
      (n-1)\% 100 - c & if $n>0 \wedge c\geq 99$\\[-2pt]
      (n+c)\% 100 - c & if $n>0 \wedge c <   99$\\[-2pt]
      0               & if $n=0$\\
    \end{cases*}$}}
 \\ \cline{2-5}
 & \texttt{\noiseddthreeonename}
 & \texttt{\noiseddthreeonekey} 
 & \gape{\makecell[l]{$f(n,c_1,c_2)=$\\
   \scalebox{0.6}{$\begin{cases*}
      f(n-1,    0,    0) + n + 300 + 20  & if $n>0 \wedge c_1\geq 100 \wedge c_2\geq 77$\\[-2pt]
      f(n-1,    0, c_2+1) + n + 300      & if $n>0 \wedge c_1\geq 100 \wedge c_2<77$\\[-2pt]
      f(n-1, c_1+1,    0) + n + 20       & if $n>0 \wedge c_1<100 \wedge c_2\geq 77$\\[-2pt]
      f(n-1, c_1+1, c_2+1) + n           & if $n>0 \wedge c_1<100 \wedge c_2<77$\\[-2pt]
      0                                  & if $n=0$\\
    \end{cases*}$}}}
 & \gape{\makecell[l]{
     \scalebox{0.7}{Long to express exactly, but}\\
     \scalebox{0.7}{for $c_1\geq 100$, $c_2\geq 77$ and $n\to\infty$,}\\
     \scalebox{0.7}{$=\frac{n(n+1)}{2}+\big(\frac{300}{101}+\frac{20}{78}\big)n + \rO(1)$}
     }}
 \\ \cline{1-5}
\multirow{6}{*}{\rotatebox[origin=c]{90}{\texttt{\catnonmonot}}}
 & \texttt{\incronename}
 & \texttt{\incronekey}  
 & \gape{\scalebox{0.7}{$f(x)=\begin{cases*}
      1+f(x+1) & if $x < 10$    \\[-2pt]
      1        & if $x \geq 10$ \\
    \end{cases*}$}}
 & $\max(1, 11-x)$
 \\ \cline{2-5}
 & \texttt{\noisystrtonename}
 & \texttt{\noisystrtonekey}  
 & \gape{\scalebox{0.7}{$f(x)=\begin{cases*}
      0        & if $x = 0    \lor  x = 20$    \\[-2pt]
      1+f(x-1) & if $x \neq 0 \land x \neq 20$ \\
    \end{cases*}$}}
 & \gape{\scalebox{0.7}{$\begin{cases*}
      x    & if $x < 20$    \\[-2pt]
      x-20 & if $x \geq 20$ \\
    \end{cases*}$}}
 \\ \cline{2-5}
 & \texttt{\memorythreename}
 & \texttt{\memorythreekey}  
 & \gape{\scalebox{0.7}{$f(i,n,s)=\begin{cases*}
      n+f(0,n,1)   & if $s = 0$                   \\[-2pt]
      1+f(i+1,n,s) & if $s > 0 \wedge i\leq n$    \\[-2pt]
      -2n          & if $s > 0 \wedge i > n$ \\
    \end{cases*}$}}
 &  \gape{\makecell[l]{
     \scalebox{0.7}{Encodes simple loop with memory leak. Sol:}\\%
     \scalebox{0.7}{$\begin{cases*}
      1      & if $s = 0$                   \\[-2pt]
      -i-n+1 & if $s > 0 \wedge i\leq n$    \\[-2pt]
      -2n    & if $s > 0 \wedge i > n$ \\
    \end{cases*}$}}}
 \\ \cline{2-5}
 & \texttt{\multiphaseonename}
 & \texttt{\multiphaseonekey}  
 & \gape{\scalebox{0.7}{$f(i,n,r)=\begin{cases*}
      0            & if $i \geq n$          \\[-2pt]
      1+f(0,n,r-1) & if $i < n \land r > 0$ \\[-2pt]
      1+f(i+1,n,r) & if $i < n \land r = 0$ \\
    \end{cases*}$}}
 & \gape{\scalebox{0.7}{$\begin{cases*}
      0   & if $i \geq n$          \\[-2pt]
      n+r & if $i < n \land r > 0$ \\[-2pt]
      n-i & if $i < n \land r = 0$ \\
    \end{cases*}$}}
 \\ \cline{1-5}
\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{\catdivandconq}}}
 & \texttt{\binsearchname}
 & \texttt{\binsearchkey} 
 & \gape{\scalebox{0.7}{$f(n) =
    \begin{cases*}
      f\Big(\Big\lfloor\frac{n}{2}\Big\rfloor\Big) + 1 & if $n > 0$ \\
      0                                                & if $n = 0$ \\
    \end{cases*}$}}
 & \gape{\scalebox{0.7}{$\begin{cases*}
      0                                 & if $n = 0$ \\[-2pt]
      1+\big\lfloor\log_2(n)\big\rfloor & if $n > 0$
    \end{cases*}$}}
 \\ \cline{2-5}
 & \texttt{\qsortonename}
 & \texttt{\qsortonekey}   
 & \gape{\scalebox{0.7}{$f(n) =
    \begin{cases*}
      f\Big(\Big\lfloor\frac{n-1}{2}\Big\rfloor\Big) + f\Big(\Big\lceil\frac{n-1}{2}\Big\rceil\Big) + n & if $n > 1$ \\
      1                                                                                                 & if $n \leq 1$ \\
    \end{cases*}$}}
 & \gape{\makecell[l]{
     \scalebox{0.7}{Hard to express exactly, but}\\
     \scalebox{0.7}{$\sim n\log_2(n)$}
     }}
 \\ \cline{2-5}
 & \texttt{\divandconqmultioneonename}
 & \texttt{\divandconqmultioneonekey} 
 & \gape{\scalebox{0.7}{$f(n) =
    \begin{cases*}
      2 f\Big(\Big\lfloor\frac{n}{3}\Big\rfloor\Big) + 5 f\Big(\Big\lfloor\frac{n}{6}\Big\rfloor\Big)+ n & if $n > 0$ \\
      1                                                & if $n = 0$ \\
    \end{cases*}$}}
 & \gape{\makecell[l]{
     \scalebox{0.7}{Hard to express exactly, but}\\
     \scalebox{0.7}{$n^{1.2764...}$}
     }}
 \\ \cline{1-5}
\multirow{3.3}{*}{\rotatebox[origin=c]{90}{\texttt{\catsuperpoly}}}
 & \texttt{\exponename}
 & \texttt{\exponekey}  
 & \gape{\scalebox{0.7}{$f(n) =
    \begin{cases*}
      2f(n-1) & if $n > 0$ \\[-2pt]
      3       & if $n = 0$ \\
    \end{cases*}$}}
 & $3\times 2^n$
 \\ \cline{2-5}
 & \texttt{\exptwoname}
 & \texttt{\exptwokey} 
 & \gape{\scalebox{0.7}{$f(n) =
    \begin{cases*}
      2f(n-1)+1 & if $n > 0$ \\[-2pt]
      3         & if $n = 0$ \\
    \end{cases*}$}}
 & $4\times 2^n - 1$
 \\ \cline{2-5}
 & \texttt{\factname}
 & \texttt{\factkey} 
 & \gape{\scalebox{0.7}{$f(n) =
    \begin{cases*}
      nf(n-1) & if $n > 0$ \\[-2pt]
      1       & if $n = 0$ \\
    \end{cases*}$}}
 & $n!$
 \\ \cline{1-5}\pagebreak
\multirow{9}{*}{\rotatebox[origin=c]{90}{\texttt{\catmisc}}}
 & \texttt{\basiconename}
 & \texttt{\basiconekey}  
 & \gape{\scalebox{0.7}{$f(n) =
    \begin{cases*}
      f(n-1)+1 & if $n > 0$ \\[-2pt]
      0        & if $n = 0$ \\
    \end{cases*}$}}
 & $n$
 \\ \cline{2-5}
 & \texttt{\sumoscname}
 & \texttt{\sumosckey}  
 & \gape{\scalebox{0.7}{$f(x,y) =
    \begin{cases*}
      f(x-1,y)   + 1 & if $x > 0 \land y > 0$ \\[-2pt]
      f(x+1,y-1) + y & if $x = 0 \land y > 0$ \\[-2pt]
      1              & if $y = 0$ \\
    \end{cases*}$}}
 & \gape{\scalebox{0.7}{$\begin{cases*}
      1                                 & if $y = 0$ \\[-2pt]
      \frac{1}{2}y^2 + \frac{3}{2}y + x & if $y > 0$ \\[2pt]
    \end{cases*}$}}
 \\ \cline{2-5}
 & \texttt{\divname}
 & \texttt{\divkey} 
 & \gape{\scalebox{0.7}{$f(x,y) =
    \begin{cases*}
      f(x-y,y) + 1 & if $x \geq y \land y > 0$ \\[-2pt]
      0            & if $x < y    \land y > 0$   \\
    \end{cases*}$}}
 & $\Big\lfloor{\frac{x}{y}}\Big\rfloor$
 \\ \cline{2-5}
 & \texttt{\nestedname}
 & \texttt{\nestedkey} 
 & \gape{\scalebox{0.7}{$f(n) =
    \begin{cases*}
      f(f(n-1)) + 1 & if $n > 0$ \\[-2pt]
      0             & if $n = 0$ \\
    \end{cases*}$}}
 & $n$
 \\ \cline{2-5}
 & \texttt{\openzipname}
 & \texttt{\openzipkey}  
 & \gape{\scalebox{0.7}{$f(x,y) =
    \begin{cases*}
      f(x-1,y-1) + 1  & if $x > 0 \land y > 0$ \\[-2pt]
      f(x,y-1)   + 1  & if $x = 0 \land y > 0$ \\[-2pt]
      f(x-1,y)   + 1  & if $x > 0 \land y = 0$ \\[-2pt]
      0               & if $x = 0 \land y = 0$ \\
    \end{cases*}$}}
 & $\max(x,y)$
 \\ \cline{2-5}
 & \texttt{\mergename}
 & \texttt{\mergekey} 
 & \gape{\makecell[l]{$f(x,y)=$\\
   \scalebox{0.7}{$\begin{cases*}
      \max(f(x-1,y), f(x,y-1)) + 1 & if $x > 0 \land y > 0$ \\[-2pt]
      0                            & if $x = 0 \lor  y = 0$ \\
    \end{cases*}$}}}
 & \gape{\scalebox{0.7}{$\begin{cases*}
      x+y-1 & if $x>0 \land y>0$ \\[-2pt]
      0     & if $x=0 \lor  y=0$ \\
    \end{cases*}$}}
 \\ \cline{2-5}
 & \gape{\makecell[l]{\texttt{\loopustarjanname}
 }} 
 & \gape{\makecell[l]{\texttt{\loopustarjankey}}}
 & \gape{\makecell[l]{$f(i,j)=$\\
   \scalebox{0.7}{$\begin{cases*}
      0                                & if $i=0$ \\[-2pt]
      1+\max(f(i-1,j+1), 1+f(i-1,j+2)) & if $i>0$
    \end{cases*}$}}}
 & \gape{\makecell[l]{
     Inlined single-function encoding\\
     of tarjan benchmark from~\cite{Sinn17-loopus,mlrec-tplp2024-preprint}\\
     $2i$ (worst-case)}}
 \\ \cline{1-5}
\end{longtable}}


==> table_of_results_all_bench.tex <==
\begin{table}[h]
\centering
\begin{adjustwidth}{-6em}{-3em}
{\scriptsize
 \setlength{\extrarowheight}{2.5pt}%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{Bench}}  
& \texttt{\prototypename}
& \texttt{\linregonlyname}
& \texttt{\ramlname}
& \texttt{\cofloconame}
& \texttt{\mathematicaname}
\\ \hline \hline
\multirow{9}{*}{\rotatebox[origin=c]{90}{\texttt{\catwithnoise}}}
& \texttt{\runningex}
& \makecell[c]{
  \phantom{.}\\[-0.8em]
  $[\ssim, \ssim]$\\
  Tight in all coeffs.,\\
  but $\rO(1)$.
  }
& \makecell[c]{
  $\snotabound$\\
  In $\frac{1}{2}n^2+\rO(n)$\\
  for $n\to\infty$
  }
& \makecell[c]{
  \phantom{.}\\[-0.8em]
  $[\ssim, \sbadub]$\\
  lb: $0.5n^2+0.5n$\\
  ub: $0.5n^2+300.5n+c$
  }
& \makecell[c]{
  \phantom{.}\\[-0.8em]
  $[\sbadlb, \sTheta]$\\
  lb: $n$\\
  ub: $2n^2+\rO(n)$
}
& $\snone$
\\ \cline{2-7}
& \texttt{\noiseddtwotwo}
& \makecell[c]{
  \phantom{.}\\[-0.8em]
  $[\ssim, \ssim]$\\
  Tight in all coeffs.,\\
  but $\rO(1)$.
  }
& \makecell[c]{
  $\snotabound$\\
  In $\sTheta(n^2)$\\
  for $n\to\infty$
  }
& \makecell[c]{
  $[\sTheta,\snone]$\\
  lb: $\sTheta(n^2)$
}
& \makecell[c]{
  \phantom{.}\\[-0.8em]
  $[\sbadlb, \sTheta]$\\
  lb: $n$\\
  ub: $302n^2+\rO(n)$
}
& $\snone$
\\ \cline{2-7}
& \texttt{\fillandfree}
&
\makecell[c]{
  \phantom{.}\\[-0.8em]
  $[\fsol-\sTheta(1), \fsol+\sTheta(1)]$\\
  $[0, 0]$     ($n=0$)\\
  $[-c, 99-c]$ ($n>0$)\\[1pt]
  }
& \makecell[c]{
  $\snotabound$\\
  ($\approx\texttt{cst}-\alpha\cdot c$)
  }
& \makecell[c]{
  $[\snone, \sbadub]$\\
  ub: $n$
  }
& \makecell[c]{
  $[\snotabound, \sbadub]$\\
  lb: $-n$\\
  ub: $n$
  }
& $\snone$
\\ \cline{2-7}
& \texttt{\noiseddthreeone}
& \makecell[c]{
  \phantom{.}\\[-0.8em]
  $[\ssim, \ssim]$\\
  Tight in all coeffs.,\\
  but $\rO(1)$.
  }
& \makecell[c]{
  $\snotabound$\\
  In $\frac{1}{2}n^2+\rO(n)$\\
  for $n\to\infty$
  }
& $[\snone, \snone]$
& $[\snone, \snone]$
& $\snone$
\\ \hline \hline
\multirow{4.7}{*}{\rotatebox[origin=c]{90}{\texttt{\catnonmonot}}}
& \texttt{\incrone}
& $[\sexactnum,\sexactnum]$
& \makecell[c]{
  $\snotabound$\\
  In $\sTheta(1)$
}
& \makecell[c]{
  \phantom{.}\\[-0.8em]
  $[\sTheta, \snone]$\\
  lb: $1$
  }
& $[\sexact, \sexact]$
& $\snone$
\\ \cline{2-7}
& \texttt{\noisystrtone}
& $[\sexactnum,\sexactnum]$
& $\sexact$
& \makecell[c]{
  \phantom{.}\\[-0.8em]
  $[\snone, \ssim]$\\
  ub: $n$
  }
& $[\sexact, \sexact]$
& \makecell[c]{
  $\ssim$/$\snotabound$\\
  ``$\exists \texttt{c},\, \fsol(n)=n+\texttt{c}$''
}
\\ \cline{2-7}
& \texttt{\memorythree}
& $[\sexactnum,\sexactnum]$
& $\sexact$
& $[\snone, \snone]$
& $[\sexact, \sexact]$
& $\snone$
\\ \cline{2-7}
& \texttt{\multiphaseone}
& $[\sexact,\sexact]$
& $\sexact$
& $[\snone, \snone]$
& $[\sexact, \sexact]$
& $\snone$
\\ \hline \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{\catdivandconq}}}
& \texttt{\binsearch}
& \makecell[c]{
    $[\sTheta, \ssim]$\\
    lb: $\approx \frac{2}{3} \log_2(n)$
  }
& \makecell[c]{
    $\snotabound$\\
    $\approx \log_2(n)$
  }
& \makecell[c]{
    $[\snone, \sbadub]$\\
    ub: $\sTheta(n)$
  }
& $[\snone, \snone]$
& \makecell[c]{
    $\snone$ without help\\
    $[\ssim, \ssim]$ with help
  }
\\ \cline{2-7}
& \texttt{\qsortone}
& $[\ssimnum, \ssim]$
& \makecell[c]{
    $\snotabound$\\
    $\approx 1.2 n\log_2(n)$
  }
& \makecell[c]{
    $[\snone, \sbadub]$\\
    ub: $\sTheta(n^2)$
  }
& $[\snone, \snone]$
& \makecell[c]{
    $\snone$ without help\\
    $[\ssim, \ssim]$ with strong help
  }
\\ \cline{2-7}
& \texttt{\divandconqmultioneone}
& \makecell[c]{
    $[\sbadlb, \sbadub]$\\
    lb: $\approx 2n\log_2(n)$\\
    ub: $\approx 1.2 n^2$
  }
& \makecell[c]{
    $\snotabound$\\
    $\approx 20 n\log_2(n)$
  }
& \makecell[c]{
    $[\sbadlb, \sbadub]$\\
    lb: $\sTheta(n)$\\
    ub: $\sTheta(n^2)$
  }
& $[\snone, \snone]$
& $\snone$
\\ \hline \hline
\multirow{7.5}{*}{\rotatebox[origin=c]{90}{\texttt{\catsuperpoly}}}
& \texttt{\expone}
& $[\sexact, \sexact]$
& $\sexact$
& \makecell[c]{
  $[\sbadlb, \snone]$\\
  lb: $\sTheta(n^d)$\\
  (Poly lb in\\selected degree)
  }
& $[\snone, \snone]$
& $\sexact$
\\ \cline{2-7}
& \texttt{\exptwo}
& $[\sexact, \sexact]$
& $\sexact$
& \makecell[c]{
  $[\sbadlb, \snone]$\\
  lb: $\sTheta(n^d)$\\
  (Poly lb in\\selected degree)
  }
& $[\snone, \snone]$
& $\sexact$
\\ \cline{2-7}
& \texttt{\fact}
& $[\sexact, \sexact]$
& $\sexact$
& \makecell[c]{
  $[\sbadlb, \snone]$\\
  lb: $\sTheta(n^d)$\\
  (Poly lb in\\selected degree)
  }
& \makecell[c]{
  $\snone$\\
  $\snotabound$ for $n\geq 2$
  }
& $\sexact$
\\ \hline \hline
& \texttt{\basicone}
& $[\sexact, \sexact]$
& $\sexact$
& $[\sexact, \sexact]$
& $[\sexact, \sexact]$
& $\sexact$
\\ \cline{2-7}
& \texttt{\sumosc}
& $[\sexact, \sexact]$
& $\sexact$
& \makecell[c]{
  $[\snotabound, \sbadub]$\\
  lb: $\frac{1}{2}y^2+\frac{3}{2}y+1$\\
  \phantom{lb: } ($\snotabound$ in $x=0$)\\
  ub: $\frac{1}{2}y^2+\frac{3}{2}y+x+1$\\
  \phantom{ub: } ($\sbadub$ in $y=0$)
  }
& \makecell[c]{
  $[\snotabound, \sbadub]$\\
  lb: $\sTheta(1)$, $\snotabound$ in $(0,1)$\\
  ub: $2y^2+xy+\rO(y)$
  }
& $\snone$
\\ \cline{2-7}
& \texttt{\divben}
& \makecell[c]{
  $[\sbadlb, \sbadub]$\\
  lb: $\sTheta(1)$\\
  ub: $\max(x-y+1,0)$
  }
& \makecell[c]{
  $\snotabound$\\
  For $x\geq y\geq 1$,\\
  $\approx 0.015x-0.025y+\rO(1)$
  }

& $[\snone, \snone]$
& \makecell[c]{
  $[\snone, \sbadub]$\\
  ub: $\max(x-y+1,0)$
  }
& \makecell[c]{
  $\snone$\\
  $\snone$ without help\\
  ``x/y'' (no int) with help
  }
\\ \cline{2-7}
\multirow{3}{*}{\rotatebox[origin=c]{90}{\texttt{\catmisc}}}
& \texttt{\nested}
& $[\sexact, \sexact]$
& $\sexact$
& $[\sexact, \sexact]$
& $[\snone, \snone]$
& $\snone$
\\ \cline{2-7}
& \texttt{\openzip}
& \makecell[c]{
  $[\sTheta, \snotabound]$\\
  Exact for $x=0\vee y=0$\\
  For $x>0\wedge y>0$,\\
  lb: $\approx \frac{1}{2}x+\frac{1}{2}y$\\
  ub: $\approx 0.99x+0.99y+\rO(1)$
  }

& \makecell[c]{
  $\snotabound$\\
  Exact for $x=0\vee y=0$\\
  For $x>0\wedge y>0$,\\
  $\approx 0.6x+0.6y+\rO(1)$
  }
& \makecell[c]{
  $[\sbadlb, \sTheta]$\\
  lb: $y$\\
  ub: $x+y$\\
  }
& $[\sexact, \sexact]$
& $\snone$
\\ \cline{2-7}
& \texttt{\mergeben}
& $[\sexactnum, \sexactnum]$
& $\sexact$
& \makecell[c]{
  $[\snone, \ssim]$\\
  ub: $x+y$\\
  }
& \makecell[c]{
  $[\sbadlb, \sexact]$\\
  lb: $\min(x, y)$\\
  (lb(bc) instead\\of lb(wc))
  }
& $\snone$
\\ \cline{2-7}
& \texttt{\loopustarjan} %
& $[\sexact, \sexact]$
& $\sexact$
& $[\snone, \sexact]$
& \makecell[c]{
  $[\sTheta, \sexact]$\\
  lb: $i$\\
  (lb(bc) instead\\of lb(wc))
  }
& $\snone$
\\ \hline
\end{tabular}}
\end{adjustwidth}
\vspace*{1em}
\caption{Experimental evaluation and comparison.\label{table:results-full}}
\end{table}



==> table_runnex_results.tex <==
\begin{table}
\centering
\footnotesize
 \setlength{\extrarowheight}{2.5pt}%
\begin{tabular}{| c | c | c |}
\hline
\texttt{\prototypename}
& \texttt{\ramlname}
& \texttt{\cofloconame}
\\ \hline
\gape{\makecell[l]{
    Upper bound:\\
    \scalebox{0.7}{$\begin{cases*}
      \frac{1}{2}n^2+\frac{701}{202}n+\frac{30000}{101}\\
           \qquad \text{ if } n>0 \wedge c\geq 100\\[-2pt]
      \frac{1}{2}n^2+\frac{701}{202}n+\frac{300}{101}c\\
           \qquad \text{ if } n>0 \wedge c <   100\\[-2pt]
      c \qquad\!\!\! \text{ if } n=0\\
    \end{cases*}$}\\
    Lower bound:\\
    \scalebox{0.7}{$\begin{cases*}
      \frac{1}{2}n^2+\frac{701}{202}n+100\\
           \qquad \text{ if } n>0 \wedge c\geq 100\\[-2pt]
      \frac{1}{2}n^2+\frac{701}{202}n+\frac{300}{101}c-\frac{19900}{101}\\
           \qquad \text{ if } n>0 \wedge c <   100\\[-2pt]
      c \qquad\!\!\! \text{ if } n=0\\
    \end{cases*}$}\\
    }}
&
\gape{\makecell[l]{
    Upper bound:\\
    $\frac{1}{2}n^2+\frac{601}{2}n+c$\\
    \phantom{.}\\
    Lower bound:\\
    $\frac{1}{2}n^2+\frac{1}{2}n$\\
    }}
&
\gape{\makecell[l]{
    Upper bound:\\
    \scalebox{0.7}{$\begin{cases*}
      2n^2+300n+100 & if $n\geq 1$\\[-2pt]
      c             & if $n=0$\\
    \end{cases*}$}\\
    \phantom{.}\\
    Lower bound:\\
    \scalebox{0.7}{$\begin{cases*}
      n & if $n\geq 1$\\[-2pt]
      c                     & if $n=0$\\
    \end{cases*}$}\\
    }}
\\\hline
  \texttt{\linregonlyname}
& \texttt{\srname}~\cite{mlrec-tplp2024-preprint}
& \texttt{\mathematicaname}
\\\hline
\gape{\scalebox{0.7}{$\begin{cases*}
      \frac{1}{2}n^2 + \frac{17747}{5166}n + \frac{1874420}{8911}\\
      \qquad \text{ if } n>0 \wedge c\geq 100\\[-2pt]
      \frac{1}{2}n^2 + \frac{12169}{3503}n + \frac{7429}{2570}c -\frac{112277}{1182}\\
      \qquad \text{ if } n>0 \wedge c <   100\\[-2pt]
      c \qquad\!\!\! \text{ if } n=0\\
    \end{cases*}$}}
&
\gape{\scalebox{0.7}{$\begin{cases*}
      \texttt{0.49929*n**2 + 3.4857*n + 222.34}\\
      \qquad \text{ if } n>0 \wedge c\geq 100\\[-2pt]
      \texttt{0.49960*n**2 + 3.6287*n + 2*c    - 66.422}\\
      \qquad \text{ if } n>0 \wedge c <   100\\[-2pt]
      \texttt{c} \qquad\!\!\! \text{ if } n=0\\
    \end{cases*}$}}
&
\texttt{None}
\\\hline
\end{tabular}
\vspace{1em}
\caption{Full results obtained by each tool for the running example.
  Results for the symbolic regression presented in~\cite{mlrec-tplp2024-preprint}
  is included for completeness: it does not manage to discover the
  exact solution either, even if floor and division nodes are allowed.
  \label{table:runnex_results}
}
\end{table}


==> tables_of_results.tex <==

\begin{table}[h]
\centering
{\footnotesize
\begin{tabular}{| c || c | c | c | c |}
\hline
Tool
& \rotatebox[origin=c]{270}{\;\;\texttt{\runningexname}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\noiseddtwotwoname}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\fillandfreename}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\noiseddthreeonename}\;\;}
\\ \hline
\texttt{\prototypename}
& \makecell[c]{
  $[\ssim, \ssim]$\\
  Tight in all coeffs.,\\
  but $\rO(1)$.
  }
& \makecell[c]{
  $[\ssim, \ssim]$\\
  Tight in all coeffs.,\\
  but $\rO(1)$.
  }
&
\makecell[c]{
  (? - TODO)\\ %
  $[0, 0]$     ($n=0$)\\
  $[-c, 99-c]$ ($n>0$)
  }
& \makecell[c]{
  $[\ssim, \ssim]$\\
  Tight in all coeffs.,\\
  but $\rO(1)$.
  }
\\ \hline
\texttt{\linregonlyname}
& \makecell[c]{
  $\snotabound$\\
  In $\frac{1}{2}n^2+\rO(n)$\\
  for $n\to\infty$
  }
& \makecell[c]{
  $\snotabound$\\
  In $\sTheta(n^2)$\\
  for $n\to\infty$
  }
& \makecell[c]{
  $\snotabound$\\
  (? - TODO)\\ %
  ($\approx\texttt{cst}-\alpha\cdot c$)
  }
& \makecell[c]{
  $\snotabound$\\
  In $\frac{1}{2}n^2+\rO(n)$\\
  for $n\to\infty$
  }
\\ \hline
\texttt{\ramlname} 
& \makecell[c]{
  $[\ssim, \sbad]$\\
  lb: $0.5n^2+0.5n$\\
  ub: $0.5n^2+300.5n+c$
  }
& \makecell[c]{
  $[\sTheta,\snone]$\\
  lb: $\sTheta(n^2)$
}
& \makecell[c]{
  $[\snone, \sbad]$\\
  ub: $n$
  }
& $[\snone, \snone]$
\\ \hline
\texttt{\cofloconame} 
& \makecell[c]{
  $[\sbad, \sTheta]$\\
  lb: $n$\\
  ub: $2n^2+\rO(n)$
}
& \makecell[c]{
  $[\sbad, \sTheta]$\\
  lb: $n$\\
  ub: $302n^2+\rO(n)$
}
& \makecell[c]{
  $[\snotabound, \sbad]$\\
  lb: $-n$\\
  ub: $n$
  }
& $[\snone, \snone]$
\\ \hline
\texttt{\mathematicaname}
& $\snone$
& $\snone$
& $\snone$
& $\snone$
\\ \hline
\end{tabular}}
\vspace*{1em}
\caption{Results for category \texttt{\catwithnoise}.}
\end{table}

\begin{table}[h]
\centering
{\footnotesize
 \setlength{\extrarowheight}{2.5pt}%
\begin{tabular}{| c || c | c | c | c |}
\hline
Tool
& \rotatebox[origin=c]{270}{\;\;\texttt{\incronename}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\noisystrtonename}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\memorythreename}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\multiphaseonename}\;\;}
\\ \hline
\texttt{\prototypename}
& $[\sexactnum,\sexactnum]$
& $[\sexactnum,\sexactnum]$
& $[\sexactnum,\sexactnum]$
& $[\sexact,\sexact]$
\\ \hline
\texttt{\linregonlyname}
& \makecell[c]{
  $\snotabound$\\
  In $\sTheta(1)$
}
& $\sexact$
& $\sexact$
& $\sexact$
\\ \hline
\texttt{\ramlname}
& \makecell[c]{
  $[\sTheta, \snone]$\\
  lb: $1$
  }
& \makecell[c]{
  $[\snone, \ssim]$\\
  ub: $n$
  }
& $[\snone, \snone]$
& $[\snone, \snone]$
\\ \hline
\texttt{\cofloconame}
& $[\sexact, \sexact]$
& $[\sexact, \sexact]$
& $[\sexact, \sexact]$
& $[\sexact, \sexact]$
\\ \hline
\texttt{\mathematicaname}
& $\snone$
& \makecell[c]{
  $\ssim$/$\snotabound$\\
  ``$\exists \texttt{c},\, \fsol(n)=n+\texttt{c}$''
}
& $\snone$
& $\snone$
\\ \hline
\end{tabular}}
\vspace*{1em}
\caption{Results for category \texttt{\catnonmonot}.}
\end{table}

\begin{table}[h]
\centering
{\footnotesize
 \setlength{\extrarowheight}{2.5pt}%
\begin{tabular}{| c || c | c | c |}
\hline
Tool
& \rotatebox[origin=c]{270}{\;\;\texttt{\binsearchname}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\qsortonename}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\divandconqmultioneonename}\;\;}
\\ \hline
\texttt{\prototypename}
& \makecell[c]{
    $[\sTheta, \ssim]$\\
    lb: $\approx \frac{2}{3} \log_2(n)$
  }
& $[\ssimnum, \ssim]$
& \makecell[c]{
    $[\sbad, \sbad]$\\
    lb: $\approx 2n\log_2(n)$\\
    ub: $\approx 1.2 n^2$
  }
\\ \hline
\texttt{\linregonlyname} 
& \makecell[c]{
    $\snotabound$\\
    $\approx \log_2(n)$
  }
& \makecell[c]{
    $\snotabound$\\
    $\approx 1.2 n\log_2(n)$
  }
& \makecell[c]{
    $\snotabound$\\
    $\approx 20 n\log_2(n)$
  }
\\ \hline
\texttt{\ramlname}
& \makecell[c]{
    $[\snone, \sbad]$\\
    ub: $\Theta(n)$
  }
& \makecell[c]{
    $[\snone, \sbad]$\\
    ub: $\Theta(n^2)$
  }
& \makecell[c]{
    $[\sbad, \sbad]$\\
    lb: $\Theta(n)$\\
    ub: $\Theta(n^2)$
  }
\\ \hline
\texttt{\cofloconame}
& $[\snone, \snone]$
& $[\snone, \snone]$
& $[\snone, \snone]$
\\ \hline
\texttt{\mathematicaname}
& \makecell[c]{
    $\snone$ without help\\
    $[\ssim, \ssim]$ with help
  }
& \makecell[c]{
    $\snone$ without help\\
    $[\ssim, \ssim]$ with strong help
  }
& $\snone$
\\ \hline
\end{tabular}}
\vspace*{1em}
\caption{Results for category \texttt{\catdivandconq}.}
\end{table}

\begin{table}[h]
\centering
{\footnotesize
\begin{tabular}{| c || c | c | c |}
\hline
Tool
& \rotatebox[origin=c]{270}{\;\;\texttt{\exponename}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\exptwoname}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\factname}\;\;}
\\ \hline
\texttt{\prototypename}
& $[\sexact, \sexact]$
& $[\sexact, \sexact]$
& $[\sexact, \sexact]$
\\ \hline
\texttt{\linregonlyname} 
& $\sexact$
& $\sexact$
& $\sexact$
\\ \hline
\texttt{\ramlname}
& \makecell[c]{
  $[\sbad, \snone]$\\
  lb: $\sTheta(n^d)$\\
  (Poly lb in\\selected degree)
  }
& \makecell[c]{
  $[\sbad, \snone]$\\
  lb: $\sTheta(n^d)$\\
  (Poly lb in\\selected degree)
  }
& \makecell[c]{
  $[\sbad, \snone]$\\
  lb: $\sTheta(n^d)$\\
  (Poly lb in\\selected degree)
  }
\\ \hline
\texttt{\cofloconame}
& $[\snone, \snone]$
& $[\snone, \snone]$
& \makecell[c]{
  $\snone$\\
  $\snotabound$ for $n\geq 2$
  }
\\ \hline
\texttt{\mathematicaname}
& $\sexact$
& $\sexact$
& $\sexact$
\\ \hline
\end{tabular}}
\vspace*{1em}
\caption{Results for category \texttt{\catsuperpoly}.}
\end{table}

\begin{table}[h]
\centering
\begin{adjustwidth}{-3em}{-3em}
{\scriptsize
\begin{tabular}{| c || c | c | c | c | c | c | c |}
\hline
Tool
& \rotatebox[origin=c]{270}{\;\;\texttt{\basiconename}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\sumoscname}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\divname}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\nestedname}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\openzipname}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\mergename}\;\;}
& \rotatebox[origin=c]{270}{\;\;\texttt{\loopustarjanname}\;\;} %
\\ \hline
\texttt{\prototypename}
& $[\sexact, \sexact]$
& $[\sexact, \sexact]$
& \makecell[c]{
  $[\sbad, \sbad]$\\
  lb: $\mathrm{\Theta}(1)$\\
  ub: $\max(x-y+1,0)$
  }
& $[\sexact, \sexact]$
& \makecell[c]{
  $[\sTheta, \snotabound]$\\
  Exact for $x=0\vee y=0$\\
  For $x>0\wedge y>0$,\\
  lb: $\approx \frac{1}{2}x+\frac{1}{2}y$\\
  ub: $\approx 0.99x+0.99y+\rO(1)$
  }

& $[\sexactnum, \sexactnum]$
& $[\sexact, \sexact]$
\\ \hline
\texttt{\linregonlyname} 
& $\sexact$
& $\sexact$
& \makecell[c]{
  $\snotabound$\\
  For $x\geq y\geq 1$,\\
  $\approx 0.015x-0.025y+\rO(1)$
  }

& $\sexact$
& \makecell[c]{
  $\snotabound$\\
  Exact for $x=0\vee y=0$\\
  For $x>0\wedge y>0$,\\
  $\approx 0.6x+0.6y+\rO(1)$
  }
& $\sexact$
& $\sexact$
\\ \hline
\texttt{\ramlname}
& $[\sexact, \sexact]$
& \makecell[c]{
  $[\snotabound, \sbad]$\\
  lb: $\frac{1}{2}y^2+\frac{3}{2}y+1$\\
  \phantom{lb: } ($\snotabound$ in $x=0$)\\
  ub: $\frac{1}{2}y^2+\frac{3}{2}y+x+1$\\
  \phantom{ub: } ($\sbad$ in $y=0$)
  }
& $[\snone, \snone]$
& $[\sexact, \sexact]$
& \makecell[c]{
  $[\sbad, \sTheta]$\\
  lb: $y$\\
  ub: $x+y$\\
  }
& \makecell[c]{
  $[\snone, \ssim]$\\
  ub: $x+y$\\
  }
& $[\snone, \sexact]$
\\ \hline
\texttt{\cofloconame}
& $[\sexact, \sexact]$
& \makecell[c]{
  $[\snotabound, \sbad]$\\
  lb: $\sTheta(1)$, $\snotabound$ in $(0,1)$\\
  ub: $2y^2+xy+\rO(y)$
  }
& \makecell[c]{
  $[\snone, \sbad]$\\
  ub: $\max(x-y+1,0)$
  }
& $[\snone, \snone]$
& $[\sexact, \sexact]$
& \makecell[c]{
  $[\sbad, \sexact]$\\
  lb: $\min(x, y)$\\
  (lb(bc) instead\\of lb(wc))
  }
& \makecell[c]{
  $[\sTheta, \sexact]$\\
  lb: $i$\\
  (lb(bc) instead\\of lb(wc))
  }
\\ \hline
\texttt{\mathematicaname}
& $\sexact$
& $\snone$
& \makecell[c]{
  $\snone$\\
  $\snone$ without help\\
  ``x/y'' (no int) with help
  }
& $\snone$
& $\snone$
& $\snone$
& $\snone$
\\ \hline
\end{tabular}}
\end{adjustwidth}
\vspace*{1em}
\caption{Results for category \texttt{\catmisc}.}
\end{table}

